GauFRe: Gaussian Deformation Fields for Real-time Dynamic Novel View Synthesis

We propose a method that achieves state-of-the-art rendering quality and efficiency on monocular dynamic scene reconstruction using deformable 3D Gaussians. Implicit deformable representations commonly model motion with a canonical space and time-dependent backward-warping deformation field. Our method, GauFRe, uses a forward-warping deformation to explicitly model non-rigid transformations of scene geometry. Specifically, we propose a template set of 3D Gaussians residing in a canonical space, and a time-dependent forward-warping deformation field to model dynamic objects. Additionally, we tailor a 3D Gaussian-specific static component supported by an inductive bias-aware initialization approach which allows the deformation field to focus on moving scene regions, improving the rendering of complex real-world motion. The differentiable pipeline is optimized end-to-end with a self-supervised rendering loss. Experiments show our method achieves competitive results and higher efficiency than both previous state-of-the-art NeRF and Gaussian-based methods. For real-world scenes, GauFRe can train in ~20 mins and offer 96 FPS real-time rendering on an RTX 3090 GPU. Project website: https://lynl7130.github.io/gaufre/index.html

==> figure/StaticSpecific.tex <==
\begin{figure}[t!]
    \centering  
    \includegraphics[width=0.8\textwidth, trim={0.0cm, .0cm, 0.0cm, 0cm}, clip]{images/StaticSpec.pdf}
    %{
    %\small
    %\begin{tabular}{>{\centering\arraybackslash}p{0.2\linewidth}*{4}{>{\centering\arraybackslash}p{0.2\linewidth}}}
    %Input & Post-activ. & Ours & TiNeuVox~\cite{TiNeuVox}
    %\end{tabular}%
    %\vspace{-1mm}
    %}%
    \caption{%\textbf{Estimating pre-activated scale significantly improves quality on dynamic objects.} \emph{Left to right:} Ground truth, estimating post-activation scale difference, estimating pre-activation scale difference, and the results of prior TiNeuVox work~\cite{TiNeuVox} that uses an MLP to directly predict the new scale for a particular timestep.
    \yl{ToDo. Draw this in a more abstract way!}}
    \label{fig:static_specific}
\end{figure}

==> figure/deformation_warping.tex <==
\begin{figure}[t!]
    \centering  
    \includegraphics[width=\textwidth, trim={0.0cm, .0cm, 0.0cm, 0cm}, clip]{images/Deformation-Warping.pdf}
    %{
    %\small
    %\begin{tabular}{>{\centering\arraybackslash}p{0.2\linewidth}*{4}{>{\centering\arraybackslash}p{0.2\linewidth}}}
    %Input & Post-activ. & Ours & TiNeuVox~\cite{TiNeuVox}
    %\end{tabular}%
    %\vspace{-1mm}
    %}%
    \caption{%\textbf{Estimating pre-activated scale significantly improves quality on dynamic objects.} \emph{Left to right:} Ground truth, estimating post-activation scale difference, estimating pre-activation scale difference, and the results of prior TiNeuVox work~\cite{TiNeuVox} that uses an MLP to directly predict the new scale for a particular timestep.
    \yl{ToDo}}
    \label{fig:defor_warp}
\end{figure}

==> figure/depth-vis.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=0.96\columnwidth, trim={0.0cm, 0cm, 21cm, 0cm}, clip]{images/depth.pdf}
\caption{\emph{Top to bottom}: The novel-view rendering and depth from our method for scenes from the NeRF-DS~\cite{yan2023nerfds} and  D-NeRF~\cite{pumarola2021d} datasets.
}
\label{fig:Depth_Vis}
\end{figure}

==> figure/order_act.tex <==
\begin{figure}[t!]
    \centering  
    \includegraphics[width=\columnwidth, trim={0.0cm, .0cm, 11.0cm, 0cm}, clip]{images/activation.pdf}
    {
    \small
    \begin{tabular}{>{\centering\arraybackslash}p{0.25\linewidth}*{4}{>{\centering\arraybackslash}p{0.2\linewidth}}}
    Input & Post-activ. & Ours & TiNeuVox~\cite{TiNeuVox}
    \end{tabular}%
    \vspace{-1mm}
    }%
    \caption{\textbf{Estimating pre-activated scale significantly improves quality on dynamic objects.} \emph{Left to right:} Ground truth, estimating post-activation scale difference, estimating pre-activation scale difference, and the results of prior TiNeuVox work~\cite{TiNeuVox} that uses an MLP to directly predict the new scale for a particular timestep. \yl{ToDo: replace with a NeRF-DS data, one gaussian}}
    \label{fig:order_act}
\end{figure}

==> figure/reb_extraexp_quali.tex <==
\begin{table}[h]
\centering
\begin{tabular}{p{0.3\linewidth}p{0.22\linewidth}p{0.22\linewidth}}
\multirow{4}{*}{%
  \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=1.07\linewidth,trim={0 0 0 0},clip]{images/toby-sit_gt.png}};
    \begin{scope}[x={(image.south east)},y={(image.north west)}]
      \draw[red,thick] (0.2,0.3) rectangle (0.7,0.55);
    \end{scope}
  \end{tikzpicture}%
} & GT & Ours \\
&\includegraphics[width=0.12\textwidth,trim={100pt 260pt 150pt 440pt},clip]{images/toby-sit_gt.png}
& \includegraphics[width=0.12\textwidth,trim={100pt 260pt 150pt 440pt},clip]{images/toby-sit_ours.png}
\\
~ & D3G & TiNeuVox \\
~ &
\includegraphics[width=0.12\textwidth,trim={100pt 260pt 150pt 442pt},clip]{images/toby-sit_D3G.png}
& \includegraphics[width=0.12\textwidth,trim={100pt 260pt 150pt 440pt},clip]{images/toby-sit_tineuvox.png}\\
\end{tabular}
\caption{Qualitative Result on Nerfies dataset.}
\label{fig:reb_extraexp_quali}
\end{table}

==> figure/results-qualitative-hypernerf.tex <==
\begin{figure}[t]
   \centering
   \vspace{-3mm}
   \begin{tabular}{p{0.15\linewidth}p{0.15\linewidth}p{0.15\linewidth}p{0.15\linewidth}p{0.15\linewidth}}
\centering GT & \centering Ours  & \centering 4DGS &  \centering EffG & \centering D3G 
\end{tabular}
    \includegraphics[width=1.0\linewidth]{images/focus_result_chicken.jpg}
    \includegraphics[width=1.0\linewidth]{images/focus_result_peel.jpg}
    \caption{\textbf{Qualitative results on the HyperNeRF dataset for dynamic Gaussian approaches.} Our method achieves comparable if not better results to 4DGS~\cite{wu20234dgaussians}, D3G~\cite{yang2023deformable} and EffG~\cite{katsumata2023efficient}.} 
    \label{fig:HyperNeRF-quali-concurrent}
\vspace{-.3cm}
\end{figure}

==> figure/results-qualitative-nerfds-gaussian.tex <==

\begin{figure}[t]
   \centering
   \begin{tabular}{p{0.15\linewidth}p{0.15\linewidth}p{0.15\linewidth}p{0.15\linewidth}p{0.15\linewidth}}
\centering GT & \centering Ours  & \centering 4DGS &  \centering EffG & \centering D3G 
\end{tabular}
    \includegraphics[width=1.0\linewidth]{images/as-gaus.png}
    \includegraphics[width=1.0\linewidth]{images/press-gaus.png}
    %\includegraphics[width=1.0\linewidth]{images/bell-gaus.png}
    \includegraphics[width=1.0\linewidth]{images/cup-gaus.png}
    \caption{\textbf{Qualitative results on the NeRF-DS dataset for dynamic Gaussian approaches.} Our method achieves comparable results to D3G~\cite{yang2023deformable}, while training and rendering much faster.}
    %\vspace{-6mm}
    %Sequences from top to bottom are \textit{Bell}, \textit{Press}, \textit{Sieve} and \textit{Sheet}. }
    \label{fig:NeRF-DS-quali-concurrent}
\end{figure}



==> table/loss.tex <==
{
\setlength{\tabcolsep}{2pt}

\begin{table}
\small
\begin{center}
\begin{tabular}{lccccc}
\toprule
%\multicolumn{6}{c}{D-NeRF~\cite{pumarola2021d} (synthetic)} \\
%\midrule
 & PSNR$\uparrow$ & MS-SSIM$\uparrow$ & LPIPS$\downarrow$ & Optim. $\downarrow$ & FPS$\uparrow$\\
\midrule
%T-NeRF~\cite{pumarola2021d} & 29.5 & 0.95 & 0.08 & $\sim$hours & - \\
%D-NeRF~\cite{pumarola2021d} & 30.0 &  0.95 & 0.07 & $\sim$hours & ? \\
%\midrule
L2 & \cellcolor{orange!25}23.7 & \cellcolor{orange!25}0.88 & \cellcolor{orange!25}0.150 & \cellcolor{orange!25}22mins & 29 \\
L1 & 23.6 & 0.88 & 0.152 & 32mins & \cellcolor{orange!25}54 \\
\midrule
Ours & \cellcolor{red!25}23.9 & \cellcolor{red!25}0.89 & \cellcolor{red!25}0.148 & \cellcolor{red!25}20mins & \cellcolor{red!25}96 \\
\bottomrule
\end{tabular}
\vspace{2mm}
\caption{\textbf{Comparison with L1 loss only, and L2 loss only.} Using our half-switching objective boosts quality and enhances efficiency.
% \yl{K-Plane: explicit model, Hexplane: slim}
% \yl{Needs to replace numbers with newly generated ones} 
% \nk{Do we want to include 4D Gaussians? Their errors are higher but running time is lower. What if we run their method for the same time as ours?}
%\yl{mention lpips matters somewhere}
%\yl{Hexplane-slim from Hexplane paper.}
}
\label{table:loss}
\vspace{-0.25cm}
\end{center}
\vspace{-0.25cm}
\end{table}

}

==> table/reb_d2nerfds_quanti.tex <==
{
\setlength{\tabcolsep}{2pt}

\begin{table}[t]
\small
\centering
\begin{tabular}{l ccc cc}
\toprule
\textbf{Table 2} & PSNR$\uparrow$ & MS-SSIM$\uparrow$ & LPIPS$\downarrow$ & Optim. $\downarrow$ & FPS$\uparrow$\\
\midrule
D$^2$NeRF &  22.7 & 0.85 & 0.189 & 6hours & 0.152 \\
Ours & \cellcolor{red!25}23.9 & \cellcolor{red!25}0.89 & \cellcolor{red!25}0.148 & \cellcolor{red!25}20mins & \cellcolor{red!25}96 \\
\bottomrule
\end{tabular}
%\caption{Metrics on Nerf-DS dataset.}
\label{tab:reb_d2nerfds_quanti}
\vspace{-0.5cm}
\end{table}
}

==> table/reb_extraexp_quanti.tex <==
{
\setlength{\tabcolsep}{2pt}

\begin{table}[h]
\resizebox{\linewidth}{!}{
\centering
\begin{tabular}{l cc c lc}
\toprule
\textbf{Table 1} & PSNR$\uparrow$  & MS-SSIM$\uparrow$   & FPS$\uparrow$  & Category & Stat/Dyn\\

\midrule
HyperNeRF  & \cellcolor{yellow!25}23.2 & \cellcolor{orange!25}0.81 & $<$1 & NeRF+MLP & \ding{55} \\ 
TiNeuVox   & \cellcolor{red!25}24.6 & 0.78 & $<$1 & NeRF+Voxel & \ding{55} \\ 
\midrule
NeuralDiff & 19.5 & 0.68 & $<$1 & NeRF+MLP & \ding{51} \\
D$^2$NeRF & 22.1 & \cellcolor{yellow!25}0.80 & $<$1 & NeRF+MLP & \ding{51} \\
\midrule
%3D-GS      &  &   &  \\ 
D3G    & 21.4 & 0.68 & \cellcolor{orange!25}8  & GS+MLP & \ding{55} \\ 
%EffGS  & 21.2 & 0.74 & \cellcolor{red!25}97 & GS+Poly & \ding{55} \\
%4DGS  & 23.69 & 0.821 & 23 \\
\midrule
Ours       & \cellcolor{orange!25}23.5 & \cellcolor{red!25}0.81  & \cellcolor{red!25}16 & GS+MLP & \ding{51} \\ 
\bottomrule
\end{tabular}
}
%\caption{Metrics on HyperNeRF-vrig dataset.}
\label{tab:reb_extraexp_quanti}
\end{table}

}
